Automated Temporal Equilibrium Analysis: Verification and Synthesis of Multi-Player Games

In the context of multi-agent systems, the rational verification problem is concerned with checking which temporal logic properties will hold in a system when its constituent agents are assumed to behave rationally and strategically in pursuit of individual objectives. Typically, those objectives are expressed as temporal logic formulae which the relevant agent desires to see satisfied. Unfortunately, rational verification is computationally complex, and requires specialised techniques in order to obtain practically useable implementations. In this paper, we present such a technique. This technique relies on a reduction of the rational verification problem to the solution of a collection of parity games. Our approach has been implemented in the Equilibrium Verification Environment (EVE) system. The EVE system takes as input a model of a concurrent/multi-agent system represented using the Simple Reactive Modules Language (SRML), where agent goals are represented as Linear Temporal Logic (LTL) formulae, together with a claim about the equilibrium behaviour of the system, also expressed as an LTL formula. EVE can then check whether the LTL claim holds on some (or every) computation of the system that could arise through agents choosing Nash equilibrium strategies; it can also check whether a system has a Nash equilibrium, and synthesise individual strategies for players in the multi-player game. After presenting our basic framework, we describe our new technique and prove its correctness. We then describe our implementation in the EVE system, and present experimental results which show that EVE performs favourably in comparison to other existing tools that support rational verification.

==> app.tex <==
\section{Proofs not in the main text}

\begin{lemma}[Goals satisfaction invariance - Lemma~\ref{lmm:satinvariance}]
	\label{app:lmm:satinvariance}
	Let $\LTLGame$ be an \LTL game and $\ParGame$ its associated parity game.
	Then, for every strategy profile $\vec{\sigma}$ and player~$i$, it is the case that $\pi(\vec{\sigma}) \models \gamma_{i}$ in $\LTLGame$ if and only if $\pi(\vec{\sigma}) \models \alpha_{i}$ in $\ParGame$.
\end{lemma}

\begin{proof}
	We prove the statement by double implication.
	To show the left to right implication, assume that $\pi(\vec{\sigma}) \models \gamma_{i}$ in $\LTLGame$, for any player~$i \in \Ag$, and let $\pi$ denote the infinite path generated by $\vec{\sigma}$ in $\LTLGame$; 
	thus, we have that~$\labFun(\pi) \models \gamma_{i}$.
	On the other hand, let $\pi'$ denote the infinite path generated in~$\ParGame$ by the same strategy profile~$\vec{\sigma}$.
	Observe that the first component of~$\pi'$ is exactly~$\pi$.
	Moreover, consider the~$(i + 1)$-th component $\rho_{i}$ of $\pi'$.
	By the definition of $\ParGame$, it holds that $\rho_{i}$ is the run executed by the automaton $\Automaton[\gamma_{i}]$ when the word $\labFun(\pi)$ is read.
	By the definition of the labelling function of $\ParGame$, it holds that the parity of~$\pi'$ according to $\alpha'_{i}$ corresponds to the one recognised by $\Automaton[\gamma_{i}]$ in $\rho_{i}$.
	Thus, since we know that~$\labFun(\pi) \models \gamma_{i}$, it follows that $\rho_{i}$ is accepting in $\Automaton[\gamma_{i}]$ and therefore $\pi' \models \alpha_{i}$, which implies that~$\pi(\vec{\sigma}) \models \alpha_{i}$ in~$\ParGame$.
	%
	For the %right to left 
	other direction, observe that all implications used above are equivalences. %Thus, 
	Using those equivalences one can reason backwards to prove the statement. 
	%\todo[color=white]{GP: Maybe we can improve the right-to-left.}
\end{proof}


\begin{theorem}[Theorem~\ref{thm:NEinvariance}]
\label{app:thm:NEinvariance}
	Let $\LTLGame$ be an \LTL game and $\ParGame$ its associated Parity game.
	Then, $\NE(\LTLGame) = \NE(\ParGame)$.
\end{theorem}
\begin{proof}
	The proof proceeds by double inclusion.
	First, assume that a strategy profile~$\vec{\sigma} \in \NE(\LTLGame)$ is a Nash Equilibrium in $\LTLGame$ and, by contradiction, it is not a Nash Equilibrium in $\ParGame$.
	Observe that, due to Lemma~\ref{lmm:satinvariance}, we known that the set of players that get their goals satisfied by~$\pi(\vec{\sigma})$ in~$\LTLGame$ (the ``winners'', $W$) is the same set of players that get their goals satisfied by~$\pi(\vec{\sigma})$ in~$\ParGame$. Then, there is player~$j \in L = \Ag \setminus W$ and a strategy $\sigma_{j}'$ such that $\pi((\vec{\sigma}_{-j}, \sigma_{j}')) \models \alpha_{j}$ in~$\ParGame$.
	Then, due to Lemma~\ref{lmm:satinvariance}, we have that $\pi((\vec{\sigma}_{-j}, \sigma_{j}')) \models \gamma_{j}$ in~$\LTLGame$ and so $\sigma_{j}'$ would be a beneficial deviation for player~$j$ in $\LTLGame$ too---a contradiction.
	On the other hand, for every $\vec{\sigma} \in \NE(\ParGame)$, we can reason in a symmetric way and conclude that $\vec{\sigma} \in \NE(\LTLGame)$.
\end{proof}


==> eve-mcmas-exp.tex <==
%\documentclass[]{article}
%\usepackage{multirow}
%
%%opening
%\title{Experiments}
%\author{}
%
%\begin{document}
%
%\maketitle
%
%%\begin{abstract}
%%
%%\end{abstract}

%\usepackage{multirow,booktabs}
%\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\setlength{\tabcolsep}{5pt}

\section{Experiments: Bisimulation Examples}\label{apdx:bisim-exp}
These experiments are taken from the motivating examples in~\cite{GHPW17}. We extended the number of states by adding more layers to the game structures used there in order to test the practical performance of \EVE, \MCMAS, and \PRALINE. The experiments were performed on a PC with Intel i7-4702MQ CPU 2.20GHz machine with 12GB of RAM running Linux kernel version 4.14.16-300.fc26.x86\_64. We divided the test cases based on the number of Kripke states and edges; then, for each case, we report (i) the total running time (``time''), (ii) whether the tools find any Nash equilibria (``NE''), and (iii) \textit{discounted execution time} (``disc.\ time''). Discounted execution time is the amount of time used after $ \mathcal{G}_{\text{PAR}} $ has been built until the tool terminates and outputs the result. This is to enable a comparison between \EVE and \PRALINE, since the latter only accepts B{\"u}chi goals (while \EVE accepts \LTL goals). 

\begin{table}[!t]
	\centering
	\caption{Example with no Nash equilibrium.}
	\label{tab:none}
	\ra{1.1}
	\begin{tabular}{@{}rrcrccrcrcrc@{}}
		\toprule
		\multirow{2}{*}{states} & \multirow{2}{*}{edges} & & \multicolumn{2}{c}{\textbf{\MCMAS}} & & \multicolumn{3}{c}{\textbf{\EVE}} &  & \multicolumn{2}{c}{\textbf{\PRALINE}} \\ \cmidrule{4-5} \cmidrule{7-9} \cmidrule{11-12}
		&		&& \multirow{2}{*}{time (s)} &  \multirow{2}{*}{NE}	&& \multirow{2}{*}{time (s)} & \multirow{2}{*}{\shortstack{disc.\\time (s)}}   & \multirow{2}{*}{NE}	&& \multirow{2}{*}{\shortstack{disc.\\time (s)}} &  \multirow{2}{*}{NE} \\
		&&&&&&&&&&&\\
		\midrule
		5	& 80	&& \textbf{0.04}& No	&& 0.75				& 0.14 			& Yes		&& 0.25 	& No\\
		8	& 128	&& \textbf{0.24}& No	&& 2.99				& 0.22 			& Yes		&& 0.54 	& No\\
		11	& 176	&& 6.28			& No	&& \textbf{4.80}	& \textbf{0.31} & Yes		&& 0.80 	& No\\
		14	& 224	&& 273.14		& No	&& \textbf{7.46}	& \textbf{0.44} & Yes		&& 1.03 	& No\\
		17	& 272	&& TO			& --	&& \textbf{13.31}	& \textbf{0.50} & Yes		&& 1.30 	& No\\
		\vdots	& \vdots&& \vdots		& \vdots&& \vdots 			& \vdots 		& \vdots 	&& \vdots	& \vdots\\
		50	& 800	&& TO			& --	&& \textbf{655.80}	& \textbf{2.58} & Yes 		&& 4.50 	& No\\
		\bottomrule
	\end{tabular}
	\centering
	\caption{Example with Nash equilibria}
	\label{tab:ne}
	\ra{1.1}
	\begin{tabular}{@{}rrcrccrcrcrc@{}}
		\toprule
		\multirow{2}{*}{states} & \multirow{2}{*}{edges} & & \multicolumn{2}{c}{\textbf{\MCMAS}} & & \multicolumn{3}{c}{\textbf{\EVE}} &  & \multicolumn{2}{c}{\textbf{\PRALINE}} \\ \cmidrule{4-5} \cmidrule{7-9} \cmidrule{11-12}
		&		&& \multirow{2}{*}{time (s)} &  \multirow{2}{*}{NE}	&& \multirow{2}{*}{time (s)} & \multirow{2}{*}{\shortstack{disc.\\time (s)}}   & \multirow{2}{*}{NE}	&& \multirow{2}{*}{\shortstack{disc.\\time (s)}} &  \multirow{2}{*}{NE} \\
		&&&&&&&&&&&\\
		\midrule
		6	& 96	&& \textbf{0.02}	& Yes	&& 1.09				& 0.12 			& Yes	&& 0.25 	& Yes\\
		9	& 144	&& \textbf{0.77}	& Yes	&& 3.36				& 0.24 			& Yes	&& 0.71 	& Yes\\
		12	& 192	&& 65.31			& No	&& \textbf{7.45}	& \textbf{0.40} & Yes	&& 1.11 	& Yes\\
		15	& 240	&& TO				& --	&& \textbf{22.24}	& \textbf{0.65} & Yes	&& 1.59 	& Yes\\
		\vdots	& \vdots&& \vdots			& \vdots&& \vdots 			& \vdots 		& \vdots&& \vdots	& \vdots\\
		51	& 816	&& TO				& --	&& \textbf{1314.47}	& \textbf{7.22} & Yes 	&& 8.89 	& Yes\\
		\bottomrule
	\end{tabular}
\end{table}

Table~\ref{tab:none} shows the results of the experiments on the example in which the model of strategies that depends only on the run (sequence of states) of the game (called run-based strategies in~\cite{GHPW17}) cannot sustain any Nash equilibria, a model of strategies that is not invariant under bisimilarity. Indeed, since \MCMAS and \PRALINE use this model of strategies, both did not find any Nash equilibria in the game, as shown in Table~\ref{tab:none}. \EVE, which uses model of strategies that, not only depends on the run of the game, but also on the actions of players (a bisimulation-invariant model of strategies called computation-based in~\cite{GHPW17}) found a Nash equilibrium in the game. We can also see that \EVE outperformed \MCMAS on games with 14 or more states. In fact, \MCMAS timed-out\footnote{We fixed the time-out value to be 3600 seconds.} on games with 17 states or more, while \EVE kept working efficiently for games of bigger size. We can also observe in the ``disc.\ time'' columns that \PRALINE performed almost as efficiently as \EVE in these experiment, although \EVE performed better in both small and large instances. 

%\begin{table}[h]
%	\centering
%	\caption{Example with no Nash equilibrium.}
%	\label{tab:none}
%	\begin{tabular}{r|r|r|l|r|l}
%		\hline
%		\multirow{2}{*}{Kripke States} & \multirow{2}{*}{Edges} & \multicolumn{2}{c}{\MCMAS} & \multicolumn{2}{c}{\EVE} \\ \cline{3-6} 
%			&		& Time (sec)&  NE	& Time (sec)& NE	\\
%		\hline
%		5	& 80	& 0.04		& No	& 0.75		& Yes	\\
%		8	& 128	& 0.24		& No	& 2.99		& Yes	\\
%		11	& 176	& 6.28		& No	& 4.80		& Yes	\\
%		14	& 224	& 273.14	& No	& 7.46		& Yes	\\
%		17	& 272	& Time-out	& -		& 13.31		& Yes	\\
%		20	& 320	& Time-out	& - 	& 24.21		& Yes	\\
%		23	& 368	& Time-out	& -		& 36.18		& Yes	\\
%		26	& 416	& Time-out 	& -		& 55.60		& Yes	\\
%		29	& 464	& Time-out	& - 	& 81.03		& Yes	\\
%		32	& 512	& Time-out	& -		& 116.14	& Yes	\\
%		35	& 560	& Time-out	& -		& 163.05	& Yes	\\
%		38	& 608	& Time-out	& -		& 225.87	& Yes	\\
%		41	& 656	& Time-out	& -		& 306.47	& Yes	\\
%		44	& 704	& Time-out	& -		& 405.45	& Yes	\\
%		47	& 752	& Time-out	& -		& 509.80	& Yes	\\
%		50	& 800	& Time-out	& -		& 655.80	& Yes 	\\
%		\hline
%	\end{tabular}
%\end{table}


%\begin{table}[t]
%	\centering
%	\caption{Example with Nash equilibria}
%	\label{tab:ne}
%	\ra{1.1}
%	\begin{tabular}{@{}rrcrccrcrcrc@{}}
%		\toprule
%		\multirow{2}{*}{states} & \multirow{2}{*}{edges} & & \multicolumn{2}{c}{\textbf{\MCMAS}} & & \multicolumn{3}{c}{\textbf{\EVE}} &  & \multicolumn{2}{c}{\textbf{\PRALINE}} \\ \cmidrule{4-5} \cmidrule{7-9} \cmidrule{11-12}
%		&		&& \multirow{2}{*}{time (s)} &  \multirow{2}{*}{NE}	&& \multirow{2}{*}{time (s)} & \multirow{2}{*}{\shortstack{disc.\\time (s)}}   & \multirow{2}{*}{NE}	&& \multirow{2}{*}{\shortstack{disc.\\time (s)}} &  \multirow{2}{*}{NE} \\
%		&&&&&&&&&&&\\
%		\midrule
%		6	& 96	&& 0.02		& Yes	&& 1.09		& 0.12 & Yes	&& 0.25 & Yes\\
%		9	& 144	&& 0.77		& Yes	&& 3.36		& 0.24 & Yes	&& 0.71 & Yes\\
%		12	& 192	&& 65.31	& No	&& 7.45		& 0.40 & Yes	&& 1.11 & Yes\\
%		15	& 240	&& TO	& --	&& 22.24	& 0.65 & Yes	&& 1.59 & Yes\\
%		\vdots	& \vdots	&& \vdots	& \vdots	&& \vdots & \vdots & \vdots && \vdots	& \vdots\\
%		51	& 816	&& TO	& --	&& 1314.47	& 7.22 & Yes 	&& 8.89 & Yes\\
%		\bottomrule
%	\end{tabular}
%\end{table}

In Table~\ref{tab:ne}, we used the example in which Nash equilibria can be sustained using run-based strategies. As shown in the table, \MCMAS found Nash equilibria in games with 6 and 9 states. However, since \MCMAS uses imperfect recall, when the third layer was added (case with 12 states in Table~\ref{tab:ne}) to the game, it could not find any Nash equilibria. Regarding running times, \EVE outperformed \MCMAS from the game with 12 states and beyond, where \MCMAS timed-out on games with 15 or more states. As for \PRALINE, it performed comparably to \EVE in this experiment, but again, \EVE performed better in all instances. 

%\begin{table}[h]
%	\centering
%	\caption{Example with Nash equilibrium.}
%	\label{tab:ne}
%	\begin{tabular}{r|r|r|l|r|l}
%		\hline
%		\multirow{2}{*}{Kripke States} & \multirow{2}{*}{Edges} & \multicolumn{2}{c}{\MCMAS} & \multicolumn{2}{c}{EVE} \\ \cline{3-6} 
%		&		& Time (sec)&  NE	& Time (sec)& NE	\\
%		\hline
%		6	& 96	& 0.02		& Yes	& 1.09		& Yes	\\
%		9	& 144	& 0.77		& Yes	& 3.63		& Yes	\\
%		12	& 192	& 65.31		& No	& 7.45		& Yes	\\
%		15	& 240	& Time-out	& -		& 22.24		& Yes	\\
%		18	& 288	& Time-out	& -		& 28.46		& Yes	\\
%		21	& 336	& Time-out	& - 	& 58.51		& Yes	\\
%		24	& 384	& Time-out	& -		& 76.60		& Yes	\\
%		27	& 432	& Time-out 	& -		& 118.13	& Yes	\\
%		30	& 480	& Time-out	& - 	& 194.90	& Yes	\\
%		33	& 528	& Time-out	& -		& 265.17	& Yes	\\
%		36	& 576	& Time-out	& -		& 358.10	& Yes	\\
%		39	& 624	& Time-out	& -		& 479.29	& Yes	\\
%		42	& 672	& Time-out	& -		& 655.45	& Yes	\\
%		45	& 720	& Time-out	& -		& 840.22	& Yes	\\
%		48	& 768	& Time-out	& -		& 1054.20	& Yes	\\
%		51	& 816	& Time-out	& -		& 1314.47	& Yes 	\\
%		\hline
%	\end{tabular}
%\end{table}



%\end{document}

